Time Series Data Mining Algorithms Towards Scalable and Real-Time Behavior Monitoring

In recent years, there have been unprecedented technological advances in sensor technology, and sensors have become more affordable than ever. Thus, sensor-driven data collection is increasingly becoming an attractive and practical option for researchers around the globe. Such data is typically extracted in the form of time series data, which can be investigated with data mining techniques to summarize behaviors of a range of subjects including humans and animals. While enabling cheap and mass collection of data, continuous sensor data recording results in datasets which are big in size and volume, which are challenging to process and analyze with traditional techniques in a timely manner. Such collected sensor data is typically extracted in the form of time series data. There are two main approaches in the literature, namely, shape-based classification and feature-based classification. Shape-based classification determines the best class according to a distance measure. Feature-based classification, on the other hand, measures properties of the time series and finds the best class according to the set of features defined for the time series. In this dissertation, we demonstrate that neither of the two techniques will dominate for some problems, but that some combination of both might be the best. In other words, on a single problem, it might be possible that one of the techniques is better for one subset of the behaviors, and the other technique is better for another subset of behaviors. We introduce a hybrid algorithm to classify behaviors, using both shape and feature measures, in weakly labeled time series data collected from sensors to quantify specific behaviors performed by the subject. We demonstrate that our algorithm can robustly classify real, noisy, and complex datasets, based on a combination of shape and features, and tested our proposed algorithm on real-world datasets.

==> chapter4.tex <==
\chapter{Hybrid Shape \& Feature Classification: Features or Shape? Tackling the False Dichotomy of Time Series Classification}

\newpage

\section{Motivation}

There are two classic approaches for time series classification in the literature: shape-based classification and feature-based classification. Shape-based classification determines the best class according to a distance measure (e.g. Euclidean distance) between the unlabeled exemplar and a set prototypes to represent the classes. Feature-based classification, on the other hand, finds the best class according to the set of features defined for the time series. These features measure properties of the time series (e.g. standard deviation, mean, complexity, fractal dimension etc.). Then the unlabeled exemplar time series is classified based on its nearest neighbor in the feature space or using a decision tree or other eager learner.
Given the existence of the two rival philosophies, which one should we use? It is possible that:

\begin{enumerate}
    \item One of the two techniques dominates for all problems. However, a quick inspection of the literature [7], or a little introspection convinces us otherwise. There are clearly problems for which one of the two approaches is much better on all classes.
    
    \item On a problem-by-problem basis, one of the techniques dominates. For example, perhaps for electrocardiograms shape is the best, but for electroencephalograms feature is the best. This seems to be the implicit assumption of most of the community [13].
    
    \item On a single problem, it might be possible that one of the techniques is better for one subset of the classes, and the other technique is better for another subset. For example, perhaps for ECGs [25][26], shape is better at distinguishing between the two classes of PVCs and VTs, but shape cannot distinguish between PVCs and VF. Whereas, some feature can tease PVCs and VF apart.
\end{enumerate}

Given this third possibility, it is clear that neither of the two techniques will dominate for some problems, but that some “combination” of both might be the best. Do such domains really exist? In fact, we believe that they are very common. For example, in Figure 1 we show an example of such problem.

As we will later show, this task of classifying chicken behavior from accelerometer data is essentially impossible to solve with a single modality of classification. The peck behavior has highly conserved shape. While the dustbathing behavior does not have a stereotypical shape, it is possible to recognize by several features, including “complexity” [15][23][28]. Moreover, we believe that many problems have this property. To consider a more familiar example, for human behavior, walking can be differentiated from running or walking-upstairs based on shape, but we surely cannot expect to separate sitting from reclining based on shape. 

In this work, we introduce a framework that can learn to choose the best classification approach for any given dataset on a class-by-class basis. If a dataset is shape “friendly” (i.e. the shape alone can classify the time series), then the framework will utilize only shape. If dataset is feature “friendly”, then the framework degenerates to feature based classification. However, if a combination of shape and feature works best for a dataset on a class-by-class basis, then the framework uses an appropriate combination of both approaches.

We will demonstrate the utility of our ideas on real-world problems and show that we can significantly out-perform rival methods that consider only one modality.

Because our underlying claim is novel, we will take the time to show an explicit numerical example. Our example is semi-synthetic for clarity, but as we will later show, highly illustrative of real-world datasets.

Suppose we have a classification problem with four classes of time series, namely Gun, NoGun, Random-noise and Random-walk as shown in Figure 2. The Gun and NoGun classes are from the classic Gun dataset of the UCR time series data mining archive [8], with 100 instances, each of  length 150 data points. We randomly selected 20 instances of each class. We generated the same number of instances, with the same length for both Random-noise and Random-walk classes.

Using the one-leave-out cross validation method, we first classified these instances using one-nearest-neighbor Euclidean distance, the results for which are shown in the form of a confusion matrix.

Table 1 shows that classification using Z-normalized Euclidean distance (i.e. shape-based classification) works well for the {Gun , NoGun} subset of this problem. However, every instance of the Random-noise class is misclassified as Random-walk. In retrospect, this is not surprising. The curse of dimensionality tells us that a random vector tends to be far from all other objects [4]. Indeed, because random vectors tend to “live” on the edge of the space, and high dimensional spaces are almost all “edge”, the distance between any two random vectors tends to be close to the diameter of the space. However, the random walks are relatively smooth, and reside towards the center of the space. Thus, the nearest neighbor for any instance in Random-noise will tend to be an instance from the Random-walk class. In contrast, consider Table 2.

Here we attempt classification using one-nearest-neighbor with the complexity feature [23]. This feature can trivially distinguish between the highly complex Random-noise class and the relatively simple Random-walk class. However, as we might expect, there is little reason to expect that complexity can differentiate between Gun and NoGun since these two classes are visually very similar.

The practical upshot of this, is that shape-based classification achieves a 29\% error-rate and feature-based classification achieves a 17\% error rate. Suppose we had an oracle meta-algorithm, which computed both the shape-based and feature-based classification, but “magically” chose the prediction of the correct algorithm. This oracle algorithm could achieve only 2.5\% error rate. 
This experiment hints at our idea. If we can have a “semi-oracle” algorithm that dynamically chooses the best classification approach at query time, and can choose better than random guessing, then we could do better than either of the single modality approaches.

\subsection{The Limit and Scope of our Claims}

on, it is worth the time to make our claim more concrete and explain why it may have escaped the community’s attention.

For shape-based classification there are many distance measures we can use to measure shape similarity, including Euclidean Distance, Dynamic Time Warping, etc. [1][7][16]. In addition, while shape-based measures are often used with a nearest neighbor classifier, they can be used with decision trees, Support Vector Machines (SVM) or even as inputs to various deep learning algorithms. Similar remarks apply to feature-based learning, where there are a plethora of features and algorithms proposed [13]. We make no claims about which combination is best for any given problem. We believe that our observations have the potential to improve any current choice possible. Concretely, our claim is limited to the following:

\textbf{Claim:} There exist datasets for which an approach that is expressive enough to consider both shape and feature, can outperform the better of using just shape or feature.

Our claim is orthogonal to which distance measure, features, or classifier is used. A practical implication of our claim is that it automatically defines the appropriate strawman to compare to. In every case, the correct comparison to our combined Shape-Feature algorithm, is the identical algorithm, but with just shape, and with just feature.

Finally, it is interesting to ask why this apparently low-hanging fruit has not been exploited before, especially given the very active research community in time series classification.

While this is speculation, we believe that an overreliance on the UCR archive may be partly to blame. The vast majority of papers on time series classification consider some improvements on some of the UCR datasets as a necessary and sufficient condition for publication [1][16]. However, as [22] recently noted, many of the datasets in the archive were created by using a shape-based measure to extract exemplars from a longer time series. Thus, it is tautological to find that shape-based measures work well on this ubiquitous benchmark. To bypass this issue, and to truly stress test our approach, in this work we will attempt classification on continuous raw unedited real-world datasets.

\section{Definitions and Notation}

We begin by defining the key terms used in this work. The data we work with is a time series.
DEFINITION 3.1. A time series T is a sequence of real-valued numbers t\_i: T\ =\ [t\_1,\ t\_2,...,\ t\_n] where n is the length of T. 
Typically, neither shape nor feature based classifiers consider the entire time series to make a prediction, but instead consider only local subsequences of the times series. 

DEFINITION 3.2. A subsequence T\_{i,m} of a time series T is a continuous subset of data points from T of length m starting at position i. T\_{i,m}\ =\ [t\_i,\ t\_{i+1},...,\ t\_{i+m-1}], 1\ \le\ i\ \le\ n\ – m + 1 .

The length of the subsequence is typically set by the user, based on domain knowledge. For example, for most human actions, ½ second may be appropriate, but for classifying transient stars, three days may be appropriate.
Our basic plan is to classify the time series using a combination of feature and shape measures. It is generally accepted that the nearest neighbor classifier is one of the best options for time series data [1]. 

DEFINITION 3.3. The nearest neighbor (nn) classifier for a time series T is an algorithm that for each query Q finds its nearest neighbor in T , and assigns Q that neighbor’s class.

In case of a shape-based classifier, the nearest neighbor is defined using either the Euclidean distance (ED) or the Dynamic Time Warping (DTW) as the distance measure. The distance between a query (i.e. an unlabeled exemplar) and all the other subsequences in the time series is stored in a vector called the distance profile.

DEFINITION 3.4. A distance profile D is a vector of distances between a given query Q and each subsequence in the time series. 

Figure 3 illustrates calculating the distance profile (D). The distance measure is the Euclidean distance between Z-normalized subsequences [18][20]. The value of the distance profile is low wherever the subsequence is highly similar to the query. In case the query Q is part of the time series, the value for the distance profile at the location of query is zero, and close to zero just before and after. To avoid such trivial matches an exclusion zone with the length of $\frac{m}{2}$ (m is the length of the query) is assumed to the left and right of the location of the query [18]. The distance profile can be computed very efficiently using the MASS algorithm [6].

\section{Our Proposed Approach}

Our task-at-hand reduces to the following steps:

\begin{enumerate}
    \item Identify the set of useful features, allowing the possibility that different classes may best be distinguished with different subsets of features (including the “feature” of shape).
    
    \item Build the K independent models, one per class.
    
    \item Set the K relevant thresholds (given the user’s class-dependent tolerance for false positives/false negatives).
    
    \item Deploy the model
\end{enumerate}

This algorithm outlined in Table 5 has two subroutines outlined in Table 3. Individual elements are motivated and explained in the following subsections.

\subsection{Identify the Features}

Instead of a global model that looks at all the features, we propose a set of K individual local models. These local binary models can be considered experts in recognizing a particular class. Because of their limited task, they can choose to only consider the features (including the ‘feature’ of shape) that best recognizes that class. The choice of which features to use is beyond the scope of this paper. Fulcher et. al. [13] presented a library of over 9000 features that can be used to quantify time series properties including the classic features such as min, max, standard deviation, etc. For simplicity, we limit the features to those that have been previously introduced in the data mining literature [14][24].

\subsection{Build the Independent Models}

We are given a time series, the set of classes describing the time series and the set of features (including the feature of shape) describing each individual class. The classification process is outlined in Table 5. 

For each class, the algorithm calls the subroutine outlined in Table 3 to compute distributions (line 2).

For every feature in the set, the subroutine computes a feature vector over the data (line 2). The feature value for each instance of the given class is saved in a list (P\_list), while the feature values for other classes are saved in another list (N\_list) (lines 3-10). We assumed an exclusion zone between each two subsequences that contain an instance. The exclusion zone is an empty region where we expect that no class exists. For example, if we used a smartwatch’s accelerometer to detect when a user takes a drag from a cigarette, we should set an exclusion zone of seven minutes, otherwise another detection surely represents the same cigarette. These exclusion window lengths can be set by common sense (especially for human activities), learned from strongly labeled data, or set using domain knowledge. For example, for the chicken dataset that we describe later, the literature suggests that two examples of pecking should be at least ¼ of a second apart [15][21].

Lines 11 and 12 calculate and return the distributions of values in P\_list and N\_list. Given these distributions, the classification algorithm calculates the probability of each class for the test data using the subroutine outlined in Table 4. For each subsequence with a certain feature value, the subroutine computes and returns the probability based on the frequency of that feature value in the distribution vectors (lines 1-15). This probability is called a local model.

Lines 7-9 (Table 5) combine the local models using the Naïve Bayes formula (4.1) to generate the combined model.


\subsection{Set the Relevant Thresholds}

For each class, we need a threshold that best defines our relative tolerance for the false positives vs. false negatives. The thresholds can be either manually adjusted by the user (static) or learned through a feedback loop (dynamic), assuming ground truth labels are available. In the dynamic case, the user may inspect the results produced by multiple runs of the algorithm and choose the threshold setting corresponding to the most desired point on the ROC curve.

\subsection{Deploy the Model}

Line 11 applies the threshold on the combined model to generate the final overarching model for each class. Formally:

The algorithm classifies the data based on this final model (lines 12-16). Subsequence starting at t is classified as C\_i if its final probability is higher for C\_{i\ }than any other classes.

\section{Empirical Evaluation}

To ensure that our experiments are reproducible, we have created a supporting website which contains all data including the codes and results [12].

\subsection{Performance Evaluation}

An overview of the two datasets is presented in Table 6. The datasets used are the real datasets which include real behaviors. The human dataset is somewhat contrived, in that the individual performed proscribed behaviors in a given order [10]. Naturally the chicken dataset is not contrived in any way.

In principle, a single behavior could have two or more possible instantiations which are semantically identical. For example, a one-pump and a three-pump handshake would both be in class handshake but have very different shapes. For simplicity, in this work we assume that there is a single way to perform a behavior. However, generalizing the code to a polymorphic dictionary is trivial.

Likewise, for simplicity, in both datasets we limit our attention to binary classification problems. However, our algorithm does not make any assumptions about the number of classes. With appropriate set of features, the model can be easily generalized to the multiclass case. In a sense, these are not true binary problems, because each dataset has an implicit Other class. In the case of the Chicken dataset, the Other class is the majority of the dataset.

Another important point is that our datasets, as we elaborate in the following sections, are both weakly labeled, meaning that every annotated region contains one or more of the specified class. In addition, there are almost certainly instances of a class outside the annotated regions which the annotator failed to label. Moreover, we do not know the exact number of instances of a class inside a region. To address this issue, we utilize the concept of Multiple Instance Learning (MIL) ‎[17]. MIL assumes each annotated region as a “bag” containing one or more instances of a class. If at least a single instance of a class is matched inside a bag, it is treated as a true positive. If no instances of the class are detected inside the bag, then the entire bag is treated as a false negative. In case an instance of class is mismatched inside a bag belonging to some other behavior, then it is treated as a false positive. Finally, if no mismatch occurs inside a bag of a non-relevant class, then the entire bag is treated as a true negative.

\subsection{Case Study: Physical Activity Dataset}

The PAMAP project (Physical Activity Monitoring for Aging People) monitors the physical activity of elderly people [10]. The dataset is comprised of long multidimensional time series, with each dimension showing a signal from an accelerometer located on a certain part of the body. Figure 4 shows examples of some of these activities. Each activity is weakly labeled, meaning that every annotated region may contain more than one behavior. For example, an instance of running may contain regions of walking and standing, as the athlete pauses briefly at an intersection or watering station etc.
For simplicity, we considered data from only one sensor (the X-axis of the accelerometer on the chest). We selected three types of activities (i.e. standing, walking and running). We picked several instances of each activity from the same subject and concatenated them together to make a long time series. Figure 5 shows the train data (of length 14,000 data points) and Figure 7(a) shows the test data (of length 14,000 data points), both created in the same way. Regions of running have been interpolated between activities only as transitions (or other class).

Using the algorithm described in Section 4, we first built the models. Figure 6 shows a visual summary of the models.

As the figure shows, each of the walking and standing activities have a dominant model, with which they can almost be distinguished from other activities. Shape-based model is dominant for walking, as walking has a well-preserved shape in the entire data set. In contrast, feature-based model can better describe standing. We could describe standing class with several features such as low variance, low amplitude, non-periodic, etc. Since “complexity” combines most of these attributes into one feature, we used it in our model.

Using this model, we classified the test data. Figure 7(b) shows a visual summary of the results. We can see that the combined model works well for this dataset. Table 7 and Table 8 present the confusion matrices for walking and standing classes.

The results in Table 7 indicate that our classification algorithm achieves 66\% precision and 100\% recall in matching instances of walking. Overall, the classifier has 80\% accuracy for the walking activity.
It is important to restate that we do not measure accuracy by the number of correct and incorrect instances of a class. Instead, we count the number of bags. More precisely, if at least one instance of a class was correctly classified inside the bag corresponding to that class, we consider that bag as a true positive. The opposite is the case for false positives. As Figure 7(b) shows, our algorithm worked visually well in classifying the instances of walking, meaning that it found almost all true positives.

The results in Table 8 indicate that our algorithm achieves 100\% recall and 100\% precision for Standing. The overall accuracy is 100\% for the Standing activity. As mentioned earlier, the correct way to compare our combined shape-feature algorithm, is to compare its results to the same algorithm, but with just shape, and with just feature. Let us see what the results would be if we use only a shape-based classifier and only a feature-based classifier for this dataset. Figure 8 shows the results.

As shown in Figure 8(b), the shape-only version found almost all instances of walking. However, it missed most instances of standing. On the other hand, with the feature-only version, the algorithm correctly classified almost all instances of standing. However, it could not distinguish walking from running (the non-class).

Table 9 compares the performance of all three models. As shown in the table, the shape-based algorithm works as well for walking as the combined algorithm. However, it is much worse for standing. In contrast, feature-based algorithm works as well for standing as the combined algorithm, while it is worse for walking. The reason why accuracy is high for walking with the feature is because the algorithm did not confuse walking with standing. However, it confused almost all instances of walking with running (false positives and false negatives), due to similar complexity profiles. Thus, the precision and recall are both zero.

\subsection{Case Study: Chicken Dataset}

We investigate the utility of our algorithm for separating distinct chicken behaviors. A healthy chicken is expected to display a set of behaviors [11] [19][21]. In this work, we only considered two of them, i.e. pecking and dustbathing. Pecking is the act of striking the ground with the beak, while dustbathing is the act of grooming by rolling in the dirt.  We used the dataset introduced into the community by [15].

The training data as illustrated in Figure 9 is a 24-hour one-dimensional time series of length 8,658,539 datapoints (Blue) with its corresponding annotations (Red). Each label corresponds to one behavior and there are regions of non-behaviors between every two behaviors.

Figure 10 shows a visual summary of the models created for the train data. Here again, one class (i.e. pecking) has a dominant shape-based model, while the other class (i.e. dustbathing) has a dominant feature-based model.

We ran our classification algorithm against two versions of the test data: a short version and a long version. The short version, illustrated in Figure 11(a) is a one-dimensional time series of length 30 minutes, inspected and labeled manually by a veterinary entomologist expert. The labels correspond to the regions where one or more instances of the same behavior occurred. Figure 11(b) shows a visual summary of the classification results.

Table 10 provides the confusion matrix for the performance of pecking. Given the results in this table, our classification model has a 57\% precision and 100\% recall in matching instances of the pecking behavior. Overall, the classifier has 63\% accuracy for the pecking.

We asked an expert to further review our results. This is what he noted about false positives: “I inspected the dataset for false positive pecking behaviors. I reviewed 90 objects manually and only 15 of them looked false positives while the rest (75) looked like good pecks which have escaped human labeling.” The 15 mentioned false positives were only in 12 bags out of 76. With this expert annotation, the updated precision, recall and accuracy of pecking are 75\%, 100\% and 84\%, respectively.

Table 11 provides the confusion matrix for the performance of dustbathing. This time, our classification model achieved a 100\% precision and 100\% recall in matching instances of the dustbathing behavior. Overall, the classifier has 100\% accuracy for dustbathing, which is a favorable result.

To demonstrate the superiority of the combined model over either of the shape and the feature-based models, let us see what the results would be, if we used only a shape-based classifier or only a feature-based classifier for this dataset. Figure 12 shows the results.

As is evident from Figure 12(b), the shape-only scenario found all instances of pecking, but it missed almost all instances of dustbathing (except one). In contrast, the feature-only scenario found all instances of dustbathing, while missing many instances of pecking. Table 12 provides a brief performance summary of all three models.

Even though recall is high for pecking in the shape-based version and for dustbathing in the feature-based version, the combined model seems to beat the other two in terms of precision and accuracy. The reason is the visibly high number of false positives and false negatives in the shape-only and feature-only models.

The long version of the test data as shown in Figure 13(a) is a 24-hour one-dimensional time series. Figure 13(b) shows a visual summary of the classification results. We did not have ground truth annotations for this dataset. The reference labels only show the estimated regions for the behaviors. Moreover, it is difficult, even for an expert, to define precisely where a behavior begins and ends. Nevertheless, it is clear that our algorithm was able to classify most instances of the behaviors in the dataset.

As shown in Figure 13(b), our labels (Green) and the reference labels (Red) are in strong agreement.

Another intuitive way to validate our results is to show that their distribution matches a normal chicken’s behaviors. Most animals have a daily recurrent pattern of activity called a “Circadian Rhythm”. We examined the existence of such pattern in our results. Figure 14 shows the frequency of each behavior in our results over the course of 24 hours, computed with a 15 minute long sliding window.

As expected, the pecking behavior has the highest overall frequency and it peaks at 10 A.M., which is the feeding time. Also, there is also almost no activities before sunrise and after the artificial light goes off (i.e. 10 P.M.). The pecking behavior is very “bursty”. This may be slightly unintuitive but is a familiar fact for anyone with experience with poultry farming.

\subsection{On the Expressiveness of Our Model}

It is fair to say that our proposed method is expressive since the only difference between our algorithm and the other two methods (i.e. shape-based classification and feature-based classification) is the way we combined those two possibilities. Nothing else has changed. Therefore, we can attribute any success only to the increased expressiveness of our model. It might happen that if we put our model in another classification method such as decision tree, it wouldn’t work as well for a certain dataset.

\section{Conclusions and Future Work}

We have shown that classifying time series using both shape and feature measures is useful for some datasets, a fact that seems underappreciated in the community. To our knowledge, all relevant works in the literature have adopted either shape-based classification or the feature-based classification approach. We have described a method to create models for different classes in a dataset based on a combination of shape and feature, and tested our proposed algorithm on real datasets from different domains. We showed that our method offers significant improvements.

==> chapter_X1.tex <==
\chapter{Miscellaneous - Time2Cluster: Clustering Time Series Using Neighbor Information}

% \setlength{\textfloatsep}{5pt}
\definecolor{darkgreen}{RGB}{0, 176, 80}
\definecolor{softgreen}{RGB}{119, 172, 48}
\definecolor{Lightred}{rgb}{1,0.92,1}
\definecolor{LightCyan}{rgb}{0.90,1,1}
\definecolor{Lightgreen}{rgb}{0.96,1,0.94}
\definecolor{Lightgray}{rgb}{0.97,0.97, 0.97}

Clustering is a prominent research area in data mining. It is essentially the process of partitioning data into meaningful groups to gain new insights into problems. Ideally this partitioning happens such that data within each cluster is similar to each other, while dissimilar to data in other clusters. Many data mining algorithms use clustering as a subroutine to solve problems in their domain \cite{ye2005method, jimenez2016modeling, lopez2012classification}.


In this work we consider time series clustering, however the phrase is ``overloaded'', and may refer to several different tasks that require very different approaches. For clarity we explicitly differentiate between three most common settings:


\begin{itemize}
    \item \textbf{Whole time series clustering:} Given a set of individual time series data, the objective is to group similar time series into the same cluster \cite{keogh2005clustering, wang2004scalable}.
    Here the individual items are assumed to have been extracted and typically normalized to have the same length. Note that the task of extracting the individual items is bypassed here, yet that is typically a much harder task than the clustering task itself. 
    
    
    \item \textbf{Calendar-Based clustering:} Here the individual items to be clustered span atomic fixed periods, perhaps one day, one week, one sol \cite{van1999cluster}. For example, the items might be electrical power demand profile curves, midnight-to-midnight. Note that once the user decides on the interval’s starting point, say Monday-Sunday vs Saturday-Friday, this task essentially reduces to the previous task.
    
    \item \textbf{Subsequence time series (STS) clustering:}
    Given a single time series, clustering is performed on extracted subsequences of the time series. In this setting, the individual items are subsequences of a longer time series, however there is no natural starting point to align the subsequence extraction. Note that we cannot simply extract all subsequences and reduce the task to whole clustering, as it has been shown that this produces meaningless results \cite{keogh2005clustering}.
\end{itemize}
    
\begin{figure}[h]
\centering
\includegraphics[scale=0.25,width=0.9\columnwidth]
{clusteringfigures/pageone.png}
\caption{The correlation coefficient between a subsequence of walking behavior (\textcolor{softgreen}{green}) and its neighbors is very low because of the phase shift between subsequences. All these subsequences describe walking behavior. \textit{Pos} denotes position in respect to the position of green subsequence.}~\label{fig:pageone}
    % \vspace{-0.5cm}
\end{figure}

The first two tasks mostly reduce to a choice of a distance measure \cite{keogh2005clustering, van1999cluster, zolhavarieh2014review}. The last task is the problem of interest in this work. We argue that it is the most difficult, but also the most useful, especially for exploratory data mining. In many applications, such as health monitoring or human/animal behavior analysis, STS clustering is crucial to understand, analyze and gain actionable useful insight into the data. 


In spite of the widespread interest in both clustering and time series data, we believe that progress in the task-at-hand has been hampered by the lack of an appropriately expressive representation to characterize the clustered structure. Most of the research in this area proposes novel distance measures or algorithms \cite{zolhavarieh2014review}, however progress in either of these areas may be of little use if we are optimizing over a limited and brittle representation.

In brief, our proposed representation allows every index of a time series to be labeled in one of $K$ classes and each index is annotated by a score that reflects our confidence in the labeling. As we will show, this more expressive representation, in conjunction with our algorithm, allows us to cluster datasets that stymie state-of-the-art algorithms. In Fig.~\ref{fig:pageone} we show one sample issue that our representation can mitigate.

With classic algorithms/representations it is often the case that a subsequence is partitioned  into one cluster and its ``close'' neighbors are partitioned into another cluster, even though they are describing the same behavior. Fig.~\ref{fig:pageone} shows a subsequence of walking behavior \textcolor{softgreen}{green} and its corresponding neighbors, along with correlations to the \textcolor{softgreen}{green} subsequence. Note that correlation coefficient between the walking subsequence and its neighbors is low (i.e. distance is large). One would expect that subsequences that are neighbors and describe the same behavior to have a high correlation coefficient (i.e. low distance) with each other, but this is not the case here. The small amount of phase shift that exists in the \textcolor{softgreen}{green} subsequence and its neighbors leads to low correlation.


\vspace{0.25 cm}
Here we outline major contributions in this work:
\vspace{0.25 cm}

\begin{itemize} 
\item We introduce a novel representation for time series clustering. Our model is expressive enough to represent sparse conserved clusters, essentially time series motifs \cite{chiu2003probabilistic}, and, at the other extreme, very dense conserved clusters, essentially time series snippets \cite{imani2018matrix}.

\item We introduce \textit{Time2Cluster} algorithm to meaningfully cluster subsequences in our representation by utilizing ``temporal locality'' information for each subsequence.
\end{itemize}

\vspace{0.25 cm}

We organize rest of the paper as follows: In Section \ref{DefinitionsandNotation} we introduce necessary notation and definitions. Section \ref{RelatedWork} reviews related works. We explain the proposed Time2Cluster algorithm, in Section \ref{Time2Cluster}. In Section \ref{ExperimentalEvaluation}, we perform empirical evaluation on diverse datasets and compare our results with different baselines. Section \ref{DiscussionandConclusions} draws conclusions and suggests directions for future work.

\section{Definitions and Notation}\label{DefinitionsandNotation}
We begin by describing necessary definitions and notation. The data type of interest is \textit{time series}:

\textbf{Time series:} A time series $T$ of length $n$ is a sequence of real-valued numbers
\[t_i:T=t_1,t_2,\ldots,t_n\]

We are primarily interested in the behavior of local regions. A local region of time series is called a \textit{subsequence}:

\textbf{Subsequence:} A subsequence $T_{i,m}$ of a time series $T$ is a continuous ordered subset of values from $T$ with length $m$ starting at position $i$.\\
    \vspace{-1em}
\[T_{i,m}=t_i,t_{i+1},\ldots,t_{i+m-1}\] where \[1\le i \le n-m+1\]

To extract subsequences from time series, we can use different \textit{stride length}:

\textbf{Stride length:} In time series data, stride length is the number of data points that we shift the position of current subsequence to extract position of the next subsequence. For example, stride of length one means if the current subsequence is located at $T_{i,m}$ where $i$ is position of the subsequence from  $T$ with length $m$, then the next subsequence is $T_{i+1,m}$ where the starting position is at $i+1$.\\

In  our  algorithm  we  define \textit{BAG} as:

\textbf{BAG:}
$BAG_{(i, m)}^{ks}$ is a continuous ordered subset of subsequences which consists of $ks$ subsequences (kernel size = $ks$) starting at position $i$ and the subsequence length of $m$.

\begin{center}
$BAG_{(i, m)}^{ks}$  = {$T_{i, m}$, $T_{i + 1, m}$, ..., $T_{i + ks - 1, m}$}
\end{center}

Kernel size is the number of subsequences that we want to consider in each BAG which we denote as $ks$. We can store distances between a subsequence of a time series with all the other subsequences from the same time series in an ordered array called \textit{distance profile} [16].

\textbf{Distance profile:} A distance profile $DP$ of a time series $T$ and a given query $T_{i,m}$ is a vector which stores \textit{dist} $(T_{i,m}, T_{j,m})$ $\forall$ $j$ $\in$ $[1, 2, ... , n {-} m + 1]$ where $m$ is the subsequence length. \textit{dist} is a function that computes z-normalized Euclidean distance between input subsequences. The z-normalized Euclidean distance and Pearson correlation are related to each other using the following equation:
\[
D = \sqrt{2m (1-\rho)}
\]

where $D$ is the z-normalized Euclidean distance, m is the subsequence length and $\rho$ is the Pearson correlation. The lower and upper bound of $D$ is equal to zero and $\sqrt{4m}$ respectively which means $\rho$ equals to one (subsequences are completely correlated) and negative one (subsequences are anti correlated), respectively. We can compute the \textit{correlation matrix} using distance profile.

\textbf{Correlation matrix:} A correlation matrix $M$ stores the Pearson correlation coefficient between all subsequences of the time series. Note that the distance profile calculates the Pearson correlation of each subsequence with the time series. This means we can compute distance profile for all subsequences of the time series and create a correlation matrix by storing each distance profile in one row of the correlation matrix.

\section{Related Work}\label{RelatedWork}
Recall that our taxonomy suggests that  clustering algorithms can be classified into three  categories of ``whole time series clustering", ``calendar-based clustering'' \footnote{Note that the ``calendar'' here does not need to be the familiar days or weeks. It can be anything that produces unambiguous cycles, for example tides or batch-cycles in batch processing.}, and ``subsequence  time series clustering".

For subsequence time series (STS) clustering we can further refine the taxonomy into three different approaches.


\begin{itemize}
    \item Shape-based clustering: This method uses raw time series data and a distance measure such as Euclidean distance (ED) to measure similarity between data. For example, in \cite{paparrizos2015k} authors introduce k-shape clustering algorithm, which is similar to K-means, and it uses cross-correlation as a distance measure.
    
    \item Feature-based clustering: In this approach various features are extracted from raw time series data, and then clustering is performed in the feature space \cite{fulcher2018feature}. One advantage of this method is reducing dimensionality of the data \cite{rasanen2009feature}. Since clustering is an unsupervised task, finding an appropriate set of features remains a challenging task.
    
    \item Model-based clustering: In this approach, raw time series is used to find parameters of some model. For example, in \cite{hallac2017toeplitz} authors used model-based clustering approach for multivariate time series data. Each cluster is defined through a Markov random field, characterizing inter-dependencies between different observations in a typical subsequence of that cluster. The authors defined each cluster as a dependency network showing the relationship between different sensors. One drawback of their method is using states for clustering the time series. For example if a time series consists of five minutes of walking and five minutes of running behaviors and the multivariate time series consists of X and Y accelerations, then there would be no change of states from walking to running behaviors and their system fails to find the two clusters correctly as we show in the empirical evaluation section. Moreover, model-based clustering can suffer from scalability issues \cite{vlachos2004indexing}.
\end{itemize}

Various distance measures are used in the three aforesaid clustering approaches. The most two common similarity measures for time series data are Euclidean distance (ED) and Dynamic time warping (DTW) distance measures. ED is more efficiently calculated, however DTW may be more robust in some domains.

Another important parameter to determine is the number of clusters K. There are various methods to find the number of clusters such as Elbow method \cite{thorndike1953belongs}, Akaike information criterion (AIC) \cite{akaike1973information}, Bayesian information criterion (BIC) \cite{schwarz1978others} or the silhouette score \cite{rousseeuw1987silhouettes}. However, the number of clusters in most of the cases depends on the application.

In subsequence time series clustering, we need to determine the appropriate window size for each subsequence. There are methods that find the best window size length \cite{madrid2019matrix}, however, in most of the applications this value is determined through expert (and possibly out-of-band) knowledge. As we show in Section \ref{Sensitivity Test}, our proposed method is robust to exact window length and a wide range of window lengths work well for most data sets.

There are different ways to measure performance of clustering algorithms such as purity, Jaccard distance, silhouette score, F1-score, and Adjusted Rand Index.

Purity is a simple way to measure quality of clustering \cite{aggarwal2004framework}. High purity is easy to achieve when the number of clusters is large. Thus, purity alone is not a very reliable quality measure.

Another measure of the performance of clustering is to compute the silhouette score \cite{rousseeuw1987silhouettes}. Silhouette score measures similarity of an object to its own cluster compared to other clusters. The silhouette score ranges from $[-1, 1]$, where a high value indicates that the object is well matched to its own cluster and poorly matched to neighboring clusters. Using silhouette score for subsequence time series clustering may be inappropriate because the distance between two subsequences of the same behavior can be very different due to phase shift effect. So, in order to use silhouette score for subsequence time series clustering, the distance measure should be chosen such that phase shift effect between subsequences can be ignored.

Another way to measure performance of clustering is using the F1-score. F1-score measures quality of any given solution with respect to the ground truth \cite{van1989towards} and has been used in many time series clustering algorithms \cite{hallac2017toeplitz, kameda2006spider, gullo2012time}.
Adjusted Rand Index (ARI) is another popular measure of clustering performance \cite{rand1971objective, hubert1985comparing, yeung2001details}. Rand Index measures similarity between two data clusters, while the Adjusted Rand Index (ARI) is the corrected-for-chance version of Rand Index. Since all datasets have ground truth assignment of clusters, we evaluate performance of clustering through F1-score and Adjusted Rand Index (ARI) metrics.

\section{Time2Cluster}\label{Time2Cluster}

In brief, Time2Cluster consists of the following steps: 
\begin{enumerate}
     \item {Computing correlation matrix
     }
     \item{Computing augmented correlation using neighborhood information for each subsequence and accordingly updating the correlation matrix
     }
     \item{Using kmean++ algorithm on the augmented correlation matrix}
      \item{Computing the confidence score}
\end{enumerate}

\vspace{0.3cm}
\textbf{Correlation matrix:} The correlation matrix is Pearson correlation coefficient between each two subsequences in the time series. Basically the correlation matrix can be written as:

\begin{equation}
M=
\begin{pmatrix}
 \rho^m_{0,0}& \rho^m_{0,1}& ...& \rho^m_{0,i}& \rho^m_{0,n}\\
 \rho^m_{1,0}& \rho^m_{1,1} & ... & \rho^m_{1,i}& \rho^m_{1,n}\\
 ...& ...& ...& ...& ...\\
 \rho^m_{j,0}& \rho^m_{j,1} & ... & \rho^m_{j,i}& \rho^m_{j,n}\\
 ...& ...& ...& ...& ...\\
 \rho^m_{n,0}& \rho^m_{n,1} & ... & \rho^m_{n,i}& \rho^m_{n,n}
\end{pmatrix}
= 
\begin{pmatrix}
 DP_0\\
 DP_1\\
 ...\\
 DP_j\\
 ... \\
 DP_n
\end{pmatrix}
\end{equation}
 
and 

\[
\rho^m_{i,j} = corr(T_{i,m}, T_{j,m})
\]

Where corr is the Pearson correlation coefficient between two subsequences of length \textit{m} starting at position $i$ and $j$. Note that $\rho^m_{i,i}$ is equal to one since each subsequence is perfectly correlated to itself. We can calculate M using distance profile $DP$ as above, where $DP_j$ is distance profile of subsequence $j$ and changing the distance to Pearson correlation by using the formula of distance profile definition in Section \ref{DefinitionsandNotation}.

There have been improvements on computing distance profile for time series efficiently \cite{yeh2016matrix, zhu2016matrix}. We use these methods to compute correlation matrix efficiently for our algorithm \cite{yeh2016matrix}.

\vspace{0.3cm}
\textbf{Augmented correlation matrix:} Due to phase shift between two subsequences that are close to each other, correlation coefficient of such subsequences would have a low value, even though the subsequences represent the same behavior. We would like to have an algorithm that gives us a high correlation coefficient if any two subsequences represent the same semantic behavior in spite of the phase shift. To understand this concept, consider some time series comprised of walking followed by running as shown in Fig.~\ref{fig:fwalk_run}. The time series represents X-acceleration data of a sensor mounted on the shoe \cite{ainsworth2000compendium}.

% \vspace{-0.3cm}
\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/walk_run.png}
  \caption{Time series of walking and running behavior corresponds to X-acceleration data.}~\label{fig:fwalk_run}
    % \vspace{-0.5cm}
\end{figure}

As hinted at in Fig.~\ref{fig:pageone}, due to existence of a phase shift between a subsequence and its neighbors (``neighbor'' in the sense of similar time index), the correlation coefficient between them is low, thus using the correlation matrix as the input for any clustering method will likely not generate correct results. An ideal clustering algorithm partitions all the walking subsequences in one cluster and all the running subsequences in another cluster, given that these are two distinct behaviors. However, if we use any classic clustering algorithms such as Kmean++ \cite{arthur2006k} with K = 2 (K is the number of clusters), we do not obtain ideal results as shown in Fig.~\ref{fig:fkmean}.

For visualization purposes, we show part of the time series from Fig.~\ref{fig:fwalk_run} with labeling of Kmean++ algorithm for walking-running time series. We show labeling results in \textcolor{red}{red} (walking) and \textcolor{blue}{blue} (running) colors. The ground truth label (\textcolor{darkgreen}{green}) consists of walking behavior for about 2.5 minutes and then followed by running behavior for about 2.5 minutes. As Fig.~\ref{fig:fkmean} shows the algorithm randomly labels each subsequence as red or blue. This means the Kmean++ algorithm produces a random transition of walking and running labels. The reason is that the correlation coefficient between each subsequence and its neighbors is low due to phase shift, which in turn makes the subsequences appear distinct from each other. However, time series are not independent and identically distributed (i.i.d) random variables, and neighbors are not independent from each other. We argue that we should take this into account when clustering time series data.


% \vspace{-0.3cm}
\begin{figure}[h]
\centering
 \includegraphics[width=\linewidth]{clusteringfigures/kmean++.png}
 \caption{top) The \textcolor{darkgreen}{green} binary vector represents the ground truth bottom) The labels of Kmean++ for walking and running subsequences are shown in \textcolor{red}{red} and \textcolor{blue}{blue} color, respectively.}~\label{fig:fkmean}
    %\vspace{-0.7cm}
\end{figure}

In this section, we introduce augmented correlation matrix which will address the aforesaid problem. We need to mitigate the phase shift effect, for which one simple solution might be that if each behavior repeats exactly after a certain period of time, we can extract subsequences with the stride length of that certain period. This approach can give us subsequences with phase shift equal to zero. However, there are only a handful of special time series for which this solution might work. One example is the pedestrian count data in Melbourne \cite{melbourne}. Since the natural subsequence length in this dataset is \textit{exactly} 24 hours, for each day we can extract one subsequence starting at 12:00 AM which means the stride length is one day. There are several reasons why this solution might not be generalizable:

\begin{itemize}

\item{Many time series data do not have an exact periodicity length for all subsequences, and there is a variation in subsequence length for many datasets. For example, given a time series corresponding to walking behavior, the gait cycle subsequences are not exactly like each other, as individual tires out or encounters an incline etc.}

\item{In some cases, even though we may have an exact subsequence length, random behaviors of the user prevent using a fixed stride length. Consider a time series of a running season. It will surely not consist of just running behavior, but contains moments when the athlete pauses to tighten her laces, or pause at a crosswalk.}

\item{Most crucially, there may be different natural subsequence lengths for different behaviors. For example in the time series of Fig.~\ref{fig:fwalking_sub}, walking cycles are about 2 seconds, whereas running cycles are about 1.8 seconds.}

\end{itemize}

Thus, we need to create a clustering representation that does not assume all subsequences of the time series have exactly the same period. Our proposed method, Time2Cluster, computes the best stride length for each subsequence and therefore we have a variable stride length for time series. To achieve this, we use Bag definitions from Section \ref{DefinitionsandNotation}.

$BAG_{(i, m)}^{ks}$ consists of a subsequence $i$ and its neighbors where $ks$ is the kernel size. We use a stride length of one to extract the next subsequence and $m$ is the subsequence length. Consider two bags of walking behavior, $BAG_{(i, m)}^{ks}$ and $BAG_{(j, m)}^{ks}$ as shown in Fig.~\ref{fig:fwalking_sub}.

We compute correlation coefficient between each two BAGs rather than two subsequences. This helps to solve the phase shift problem. The correlation coefficient between $BAG_{i,m}^{ks}$ and $BAG_{j,m}^{ks}$ can be computed by calculating correlation coefficient between subsequences of two BAGs and then finding maximum correlation between the two BAGs.

At a high level, each BAG contains different subsequences with different phase shifts for one behavior, so if two BAGs contain the same behavior, then the correlation coefficient between two BAGs would be high and otherwise would be low. We can use Max pooling of size $ks \times ks$ to compute correlation coefficient between two BAGs.

Max pooling is a ``downscaling'' operation that calculates maximum value in each region. The correlation coefficient between $BAG_{i,m}^{ks}$ and $BAG_{j,m}^{ks}$ can be seen as:

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/bags.png}
  \caption{Contents of $BAG_i$ and $BAG_j$. Each $BAG$ contains one behavior but different subsequences of the same behavior (different phase shifts). Comparing two $BAG$s is meaningful because allows us to compare different behaviors, since each $BAG$ contains different phase shifts of one behavior.}~\label{fig:fwalking_sub}
    % \vspace{-0.5cm}
\end{figure}


\begin{figure}[h]
\begin{tikzpicture}

  \matrix (m)[matrix of math nodes,{left delimiter=[},{right delimiter=]}] {
   \rho^m_{0,0}& \rho^m_{0,1}& ...& \rho^m_{0,i}& ... & \rho^m_{0,n}\\
 \rho^m_{1,0}& \rho^m_{1,1} & ... & \rho^m_{1,i}& ... & \rho^m_{1,n}\\
 ...& ...& ...& ...& ...& ...\\
 \rho^m_{j,0}& \rho^m_{j,1} & ... & \rho^m_{j,i}& ... & \rho^m_{j,n}\\
 ...& ...& ...& ...& ... & ...\\
 \rho^m_{n,0}& \rho^m_{n,1} & ... & \rho^m_{n,i}& ... & \rho^m_{n,n}\\
  } ;

  \draw [red,fill=magenta!50, opacity=0.5] (m-5-3.south west) rectangle (m-3-5.north east);
  
  \node (fv) [right of=m, node distance=5cm] {Correlation between};%4.2,-1.1
  \node[text width=6cm] at (6.5,-1.4) {$BAG_i$ and $BAG_j$ is equal to max pooling of the red matrix};
  \draw[magenta, thick,->, >=,-{Stealth}] (fv) to (m-3-4.south);

\end{tikzpicture}
\end{figure}



which is related to Max pooling (M, $ ks \times ks $) where M is the correlation matrix and $ks$ is the kernel size.


Fig.~\ref{fig:faugmented_kmean} shows the result of using augmented correlation matrix for clustering of walking and running time series shown in Fig.~\ref{fig:fwalk_run}. As shown in Fig.~\ref{fig:faugmented_kmean} using augmented correlation as an input to the Kmean++ clustering algorithm generates correct results. Using BAGs instead of subsequences helps with assigning subsequences and their neighbors to the same cluster and forms a temporal consistency. 

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/augmented_kmean++.png}
  \caption{top) The \textcolor{darkgreen}{green} vector represents the ground truth bottom) Clustering walking and running behaviors using Time2Cluster algorithm using \textcolor{red}{red} and \textcolor{blue}{blue} colors, respectively.}~\label{fig:faugmented_kmean}
    %  \vspace{-0.1cm}
\end{figure}



\textbf{Confidence Score:} In the last step, we compute confidence score for each label.
This score indicates confidence of the result of Time2Cluster algorithm for each label. 
We compute the confidence score for each index $i$ by summing up the augmented correlation coefficient at index $i$ for all neighbors of index $i$ that are clustered as in the same class.
The confidence score is a real number between zero and one. A score of one for index $i$ means we are very confident about the label of that index, while a score of zero means, that the labels are probably random. 


Suppose we add random noise to the time series of walking/running activity as shown in Fig.~\ref{fig:fconfidence_score}. The Time2Cluster algorithm labels the walking behavior in one cluster (\textcolor{red}{red} part of time series) and the running and noise in another cluster (\textcolor{blue}{blue} part of time series). However as shown in Fig.~\ref{fig:fconfidence_score} the confidence score gives a high value for the labels of the walking and running activity and a low value for the noisy part of the data. 


\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/confidence_score.png}
  \caption{top) The confidence score bottom) Time series of walking/running/random noise. The \textcolor{red}{red} and \textcolor{blue}{blue} colors show the clustering results for Time2Cluster algorithm. }~\label{fig:fconfidence_score}
    %  \vspace{-0.7cm}
\end{figure}



\subsection{Time Complexity}
Computing correlation matrix takes $O(n^2)$ and time complexity of Kmean++ is $O(nK)$ where $K$ is the number of clusters, so the time complexity of Time2Cluster is $O(n^2)$.




\section{Experimental Evaluation}\label{ExperimentalEvaluation}
In this section, we demonstrate our framework through a series of experiments. To ensure that our experiments are easy to reproduce, we have created a website that contains all data/code/raw spreadsheets for all the experiments \cite{time2clusterwebiste}. To measure the performance, we fix the number of clusters for our algorithm and all baseline algorithms and evaluate clustering performance by measuring two different scores:
\begin{itemize}
    \item \textbf{Macro-F1 score} In order to compute Macro-F1 score, first for each cluster we compute F1 score which is the harmonic mean of the precision and recall as follows:

    \begin{equation}
        \frac{1}{F1} = \frac{1}{2} (\frac{1}{Precision} + \frac{1}{Recall})
    \end{equation}
 
    Then we compute Macro-F1 score which is the average of F1-score for all clusters. F1-score and Macro-F1 score are in the range of [0, 1] with F1-score equal to one means perfect clustering.
    
    \item \textbf{Adjusted Rand Index score} We further compute Adjusted Rand Index score measuring the agreement between two clusters by considering all pairs of samples, and counting pairs that are assigned to the same or different clusters in the predicted and true clusters \cite{rand1971objective, hubert1985comparing}.
    The value of Adjusted Rand Index (ARI) score is in the range of [-1, 1] with ARI score equal to one means a perfect clustering and a negative ARI score means agreement is even worse than what is expected from a random result.
\end{itemize}

\subsection{Chicken Behavior}\label{Chicken Behavior}

Poultry farms are a vital source of food to humans and the task of studying chicken behaviors is important towards improved production levels and chicken welfare \cite{tixier2011chicken}. It is believed that frequency and timing of behaviors such as pecking, preening and dustbathing can be good indicators of chicken health \cite{abdoli2018time}. Pecking refers to act of chicken striking at the ground with its beak for feeding purposes; while, cleaning and aligning of feathers with the beak is referred to as preening \cite{daigle2014moving}. Finally, the act of laying on the ground and rolling dust into the feathers is called dustbathing. Fig.~\ref{fig:pp} shows instances of pecking and preening behaviors.

\vspace{-0.5cm}
\begin{figure}[h]
\centering
  \includegraphics[width=.8\linewidth]{clusteringfigures/pp.png}
  \caption{An instance of preening (left) and pecking (right) behavior.}~\label{fig:pp}
  \vspace{-0.3cm}
\end{figure}


Fig.~\ref{fig:peck_preen_chicken} shows a time series of chicken data beginning with pecking behavior followed by preening behavior. The \textcolor{darkgreen}{green} binary vector shows the ground truth for chicken data. Using clustering can help us to analyze, understand and extract useful information from this data set. The result of Time2Cluster algorithm on chicken data set is as the following.


\begin{figure}[h]
\centering
 \includegraphics[width=\linewidth]{clusteringfigures/peck_preen_chicken.png}
  \caption{top) The \textcolor{darkgreen}{green} binary vector represents ground truth for chicken behavior bottom) Time series corresponding to X axis of chicken data.}~\label{fig:peck_preen_chicken}
    %  \vspace{-0.2cm}
\end{figure}





\begin{center}
\begin{tabular}{|c|c|}
\hline
Macro-F1 score & Adjusted Rand Index score 
    \\ \hline
   0.90 &  0.65\\ \hline
\end{tabular}
\end{center}

We also compare our results for the chicken dataset with other baselines as shown in Table\ref{tab:clustering}. For visualization purposes, we embed the data into two-dimensional space using the principal component analysis (PCA) \cite{friedman2001elements}, as shown in Fig.~\ref{fig:fpca}. As we can see in Fig.~\ref{fig:fpca}, our algorithm is successful in separating two clusters.

\vspace{-0.1cm}
\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/pca.pdf}
  \caption{Applying the principal component analysis on the augmented correlation matrix generated by Time2Cluster algorithm.}~\label{fig:fpca}
     \vspace{-0.2cm}
\end{figure}

\subsection{Human Behavior}\label{Human Behavior}
We use PAMAP physical activity monitoring dataset \cite{ainsworth2000compendium}; which contains a wide range of everyday household and fitness activities performed by a number of subjects. The data is generated by subjects wearing 3D inertial measurement units (IMUs) and a heart rate (HR) monitor. This dataset has been used for many other tasks such as activity recognition, segmentation, feature extraction, and classification.

Consider a time series that represents training session of a soccer player. The player initially warms up with exercises such as walking and running, and then she starts to play soccer. Fig.~\ref{fig:fplayingsoccer} shows a time series consisted of walking, running, and finally playing soccer from a hip-mounted accelerometer collected at 100 HZ. The Boolean vector in \textcolor{darkgreen}{green} represents the ground truth labels. 


\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/walk_run_playspoccer_pamap.png}
  \caption{top) The \textcolor{darkgreen}{green} vector represents the ground truth. bottom) Z axis of walking/running/playing soccer activities time series.}~\label{fig:fplayingsoccer} 
    % \vspace{-0.5cm}
\end{figure}

In this experiment we fix the window size to one second, and number of clusters to three. We measure performance of the Time2Cluster algorithm using Macro-F1 score and Adjusted Rand Index score. The results are shown in below.

\begin{center}
\begin{tabular}{|c|c|}
\hline
Macro-F1 score &  Adjusted Rand Index score 
    \\ \hline
   0.93 &  0.87\\ \hline
\end{tabular}
\end{center}

Our results are superior to the baseline algorithms as in Table \ref{tab:clustering}. The reason is that most of baseline algorithms cannot distinguish between superficially similar walking and running behaviors, whereas some other baseline algorithms cannot find the correct cluster for playing soccer because it comprises of a truly diverse set of behaviors.

In the next experiment, we consider a stair workout exercise  which consists of climbing stairs up and down two times. The time series and ground truth label for stair workout are shown in Fig.~\ref{fig:fstairworkout}. 

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/asc_desc_pamap.png}
  \caption{top) The \textcolor{darkgreen}{green} binary vector represents ground truth labels for the stair workout. bottom) Z axis of the stair workout time series.}~\label{fig:fstairworkout}

\end{figure}

\begin{samepage}
The result for Time2Cluster algorithm is shown in below.

\begin{center}
\begin{tabular}{|c|c|}
\hline
Macro-F1 score & Adjusted Rand Index score 
    \\ \hline
   0.82 &  0.41\\ \hline
\end{tabular}
\end{center}
\end{samepage}

For visualization purposes, we show the labeling results for Time2Cluster algorithm and different baseline algorithms in Fig.~\ref{fig:flabels}. As we can see, Time2Cluster most closely models the ground truth, whereas the results for other methods like GMM and Kshape appear essentially random.  The TICC method fails to find two clusters and simply reports most of the data points in one cluster (reports a few data points as the second cluster).

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/labels.png}
  \caption{Stair workout time series, the binary vector represents ground truth label shown in \textcolor{darkgreen}{green}. Labeling results for Time2Cluster and selected baseline algorithms.}~\label{fig:flabels}
    % \vspace{-0.5cm}
\end{figure}

\subsection{Tilt Table}\label{TiltTable}

The tilt table test is a simple, noninvasive and informative test as a diagnostic tool for patients with neurally mediated syncop, among other uses. Neurally mediated syncope refers to loss of consciousness caused by abnormality of blood pressure regulation \cite{heldt2003circulatory, heldt2004computational, goldberger2000physiobank}.


During the tilt table test, an intravenous (IV) line is placed in the patient's arm and ECG wires are attached to their chest. The patient is asked to lie flat (Fig.~\ref{fig:ftiltimage} top) and after some point, the table is tilted upright and the patient will remain in this position while his heart rate and blood pressure are monitored during the entire experiment (Fig.~\ref{fig:ftiltimage} bottom).

\begin{figure}[h]
\centering
  \includegraphics
%   [width=1.5in, height=1.3in]
  [scale=0.35]
  {clusteringfigures/tilt_image_2.pdf}
  \caption{An instance of the ABP signal when the patient is in Supine, and Upright positions. }~\label{fig:ftiltimage}
%   \vspace{-0.3cm}
\end{figure}

The dataset for tilt table is shown in Fig.~\ref{fig:ftilttable}. We use the arterial blood pressure (ABP) signal to find clusters in the time series. The ABP signal is a key source of information for determining hemodynamic state of the patient. 

As shown in Fig.~\ref{fig:ftilttable},
the clustering result of Time2Cluster algorithm is very similar to the ground truth label. Let us revisit the confidence score for Time2Cluster algorithm as we explained in Section \ref{Time2Cluster}. Note, the confidence score of all labels is high (close to one) except for a small region. The reason is that the original data contains a small region in which the sensor failed to record physiological data, and instead reported a square-wave calibration signal \cite{samaniego2003electrocardiographic}. 

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/tilttable_2.png}
  \caption{top) The confidence score (pink), labeling of Time2Cluster algorithm (purple) and ground truth (green), respectively. bottom) Time series of arterial blood pressure (ABP) signal during the tilt table test.}~\label{fig:ftilttable}
%   \vspace{-0.5cm}
\end{figure}

The result for Time2Cluster algorithm is shown in below.

\begin{center}
\begin{tabular}{|c|c|}
\hline
Macro-F1 score & Adjusted Rand Index score 
    \\ \hline
   0.97 &  0.90\\ \hline
\end{tabular}
\end{center}


In the next two Sections \ref{NumberofClusters} and \ref{Sensitivity Test}, we show how to tune user-defined parameters such as number of clusters and window size for Time2Cluster algorithm.

\subsection{Number of Clusters}\label{NumberofClusters}

In most clustering algorithms the desired number of clusters is a user-defined parameter that must be provided as an input to the clustering algorithm. However, there are auxiliary methods such as Elbow method \cite{thorndike1953belongs}, Akaike information criterion (AIC) \cite{akaike1973information, aho2014model}, and Bayesian information criterion (BIC) \cite{schwarz1978others} to help determine the number of clusters given a dataset. 

The Elbow (or knee) method is a heuristic technique that has been used in many clustering tasks \cite{bholowalia2014ebk, syakur2018integration, yao2017trajectory}. This technique consists of plotting the percentage of variance as a function of the number of clusters, and picking the elbow (i.e. sharpest point of the curve) as the natural number of clusters in the data. We can use sum of squared distance from each point to its assigned center as the percentage of variance.

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/elbow.png}
  \caption{Using Elbow method for determining the number of clusters.}~\label{fig:felbow}
%   \vspace{-0.5cm}
\end{figure}

Here we used Elbow method to determine the number of clusters for walking/running/playing soccer activities time series as shown in Fig.~\ref{fig:felbow}. As we can see, the method suggests $K = 3$ as the number of clusters. However, we acknowledge that reading an elbow curve can be somewhat subjective. 

\subsection{Sensitivity Test}\label{Sensitivity Test}
In this section, we examine the effect of window size on Time2Cluster algorithm. We repeat all the experiments of Section \ref{ExperimentalEvaluation} and use a varying window size within the range of $\sim\%50$ to $\sim\%200$ of the original window size, recomputing the Macro-F1 score.

Empirically, we find that Time2Cluster algorithm is not particularly sensitive to the window size and works well for a large range of window sizes. For example, for the walking/running/playing soccer experiment changing the window size from 75 points to 200 points, varies Macro-F1 score  from 0.77 to 0.81. The results are shown in Fig.~\ref{fig:ff1-window}.  



\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/f1-window.png}
  \caption{Computing Macro-F1 score for variable window sizes in different experiments.}~\label{fig:ff1-window}
%   \vspace{-0.5cm}
\end{figure}


\subsection{Comparing different baselines}\label{Comparing different base lines}

We use multiple clustering algorithms as the baseline \cite{tslearn, hallac2017toeplitz} to compare with our algorithm. The baseline algorithms are as following:

\begin{itemize}
    \item TICC \cite{hallac2017toeplitz}: Toeplitz Inverse Covariance-based Clustering
    \item DBA Kmeans \cite{petitjean2011global}: DTW Barycenter Averaging
    % \item Soft DTW Kmeans \cite{cuturi2017soft}: a Differentiable Loss Function for Time-Series
    \item Global Alignment Kernel Kmeans \cite{dhillon2004kernel}: Identifying nonlinear separable clusters using $K$ kernels
    \item GMM \cite{banfield1993model} : Clustering using a Gaussian Mixture Model
    \item Kshape \cite{paparrizos2015k}: Shape-based time series clustering algorithm
    \item Euclidean Kmeans: The standard Kmean clustering using Euclidean distance measure
\end{itemize}

For all the methods except TICC we fix the window size and compute the same performance measures of Macro-F1 score and Adjusted Rand Index score. For TICC algorithm we choose very smaller window size because of scalability issues (the computational time exceeds a week) and report the best performance.

As shown in Table \ref{tab:clustering}, Time2Cluster significantly outperforms the baseline algorithms. On average Time2Cluster has a Macro-F1 score of 0.91 and Adjusted Rand Index score of 0.70. In some experiments there is a huge gap between Time2Cluster and baselines performance. For example, in walking/running/playing soccer experiment the highest performance of Macro-F1 score among the baselines is 0.41 which is significantly lower than 0.93 for Macro-F1 score of Time2Cluster.



\begin{table*}[t]
\centering
\linespread{1}            
\rmfamily  
\begin{tabular}{|l||*{4}{c|}}\hline
\backslashbox[1mm]{Method}{Dataset}
&\makebox[5.5em]{Walk-Run-Play}&\makebox[5.5em]{Stair-Workout}&\makebox[5.5em]{Chicken}
&\makebox[5.5em]{Tilt Table}\\\hline\hline
\hline
  \rowcolor{Lightgreen}\multicolumn{5}{|l|}{\textbf{Macro-F1 score}} \\
 \hline
Time2Cluster & \textbf{0.93} & \textbf{0.82} & \textbf{0.90} & \textbf{0.97}  \\ %\hline
TICC \cite{hallac2017toeplitz}& 0.24 & 0.34 & 0.74 & 0.81 \\ %\hline

DBA Kmeans \cite{petitjean2011global} & 0.32 & 0.52 & 0.68 & 0.42  \\ %\hline
% Kernel Kmeans 
Global Alignment \cite{dhillon2004kernel} & 0.25 & 0.51 & 0.55 & 0.62 \\ %\hline
GMM \cite{banfield1993model} & 0.34 & 0.59 & 0.87 & 0.51 \\ %\hline
Kshape \cite{paparrizos2015k} & 0.41 & 0.67 & 0.73 & 0.44 \\ %\hline
Euclidean Kmeans  & 0.40 & 0.60 & 0.75 & 0.44 \\ \hline
 \hline\hline
\rowcolor{LightCyan} \multicolumn{5}{|l|}{\textbf{Adjusted Rand Index (ARI) score}} \\
 
 \hline
 Time2Cluster & \textbf{0.87} & \textbf{0.41} & \textbf{0.65} & \textbf{0.90}  \\ %\hline
TICC \cite{hallac2017toeplitz}& 0.005 & 0.001 & 0.28 & 0.42 \\ %\hline

DBA Kmeans \cite{petitjean2011global} & 0.06 & 0.004 & 0.13 & 0.001  \\ %\hline
% Kernel Kmeans
Global Alignment \cite{dhillon2004kernel} & 0.01 & 0.002 & 0.01 & 0.08  \\ %\hline
GMM \cite{banfield1993model} & 0.07 & 0.04 & 0.56 & 0.004  \\ %\hline
Kshape \cite{paparrizos2015k} & 0.19 & 0.12 & 0.22 & 0.001  \\ %\hline
Euclidean Kmeans  & 0.19 & 0.05 & 0.25 & 0.001  \\\hline
\end{tabular}


% \rowcolor{LightCyan} \multicolumn{5}{|l|}{\textbf{Adjusted Rand Index (ARI) score}} \\
 
%  \hline
%  Time2Cluster & \textbf{0.87} & \textbf{0.41} & \textbf{0.65} & \textbf{0.90}  \\ %\hline
% TICC \cite{hallac2017toeplitz}& 0.0005 & 0.00001 & 0.28 & 0.42 \\ %\hline

% DBA Kmeans \cite{petitjean2011global} & 0.06 & 0.004 & 0.13 & -0.04  \\ %\hline

% Global Alignment Kernel Kmeans \cite{dhillon2004kernel} & 0.01 & 0.0002 & 0.01 & 0.076732  \\ %\hline
% GMM \cite{banfield1993model} & 0.07 & 0.035 & 0.56 & 0.004  \\ %\hline
% Kshape \cite{paparrizos2015k} & 0.19 & 0.12 & 0.22 & -0.03  \\ %\hline
% Euclidean Kmeans  & 0.19 & 0.05 & 0.25 & -0.03  \\\hline


\caption {Comparing Time2Cluster with different clustering algorithms using four different datasets. We use Macro-F1 score and Adjusted Rand Index (ARI) score to report performance of each clustering algorithm.} \label{tab:clustering} 
\end{table*}

\subsection{Robustness Test}\label{Robustness Test}
In this section, we examine robustness of Time2Cluster to the effect of adding random spikes (and their inverse, i.e. dropouts) to the data. Spikes are unexpectedly rapid changes in a time series that can happen for a variety of reasons. They can be physically meaningful, but they are often the result of electronic noise. This test is designed to show how well different algorithms can cope with outliers or anomalies. We use time series of Section \ref{TiltTable}, and repeat the same experiments but this time adding increasing numbers of spikes to the time series while computing the Macro-F1 score. We also repeat this experiment for baselines algorithms that have high Macro-F1 scores in Section \ref{TiltTable}. We repeat each experiment 50 times and report the average number for each algorithm. The results are shown in Fig.~\ref{fig:ff1-spike}.

As we can see in Fig.~\ref{fig:ff1-spike}, Time2Cluster algorithm is robust to the addition of random spikes in the data. The reason is that Time2Cluster algorithm computes the correlation coefficient of different BAGs, and because each BAG contains many subsequences without spike (we are replacing few data points of time series with spikes), the algorithm tends to ignore subsequences with spikes. Spiky subsequences generate low correlation coefficient with subsequences without spikes and using max pooling can help the algorithm to ignore spiky subsequences. Also, note that with the exception of TICC algorithm, other baselines are also robust to the effect of spikes, however their Macro-F1 score is very low compared to Time2Cluster algorithm.

\begin{figure}[h]
\centering
  \includegraphics[width=\linewidth]{clusteringfigures/f1-spike.png}
  \caption{Adding different percentages of spikes to time series data and computing Macro-F1 score.}~\label{fig:ff1-spike}
%   \vspace{-0.5cm}
\end{figure}


\subsection{Speed Test}\label{speed Test}
We measured the run time for Time2Cluster algorithm in comparison to baseline algorithms as shown in Table \ref{tab:computingTime}. We report the average run time for all datasets from Section \ref{ExperimentalEvaluation}.


\begin{table}[h]
    \centering
    \linespread{1}            
\rmfamily  
    \begin{tabular}{|c|c|}
\hline
 \rowcolor{Lightgreen}\multicolumn{2}{|l|}{\textbf{Computing Time (Seconds) }} \\ \hline
Time2Cluster &  80\\%\hline
GMM & 3\\ %\hline
DBA Kmeans & 2442\\ %\hline
Kshape & 37\\ %\hline
Global Alignment Kernel Kmeans & 30949\\ %\hline
Euclidean Kmeans & 56 \\ \hline
\end{tabular}
\caption {Computing time for Time2Cluster and different baseline algorithms.}
\label{tab:computingTime}
\end{table}


The fastest algorithm is GMM, however this method often fails if the dimensionality of the problem is high. Despite the speed of GMM algorithm, as shown in Table \ref{tab:clustering} the results are poor for some of the datasets. The reason is that GMM does not take into account the spatial relationship between neighboring subsequences \cite{nguyen2011gaussian}. In order to account for spatial relationship between neighbors one can use TICC \cite{hallac2017toeplitz} method, however this method is computationally expensive for large window sizes (the computational time exceeded a week for all datasets). Besides GMM, Time2Cluster is among the fastest algorithms, on average taking about 1.5 minutes, and in terms of performance is superior to the baseline algorithms.




\section{Discussion and Conclusions}\label{DiscussionandConclusions}

We have introduced Time2Cluster, an expressive representation/algorithm for clustering time series subsequences. Our method is a shape-based clustering algorithm that is invariant to phase shift effects, allowing us to find meaningful clusters where other algorithms struggle. We demonstrated that our method is robust to a portion of data containing outliers. Moreover, we demonstrated that our method is not brittle to the exact subsequence length specified by the user, producing similar results for different window sizes. 

In future work we will investigate pruning, indexing and early abandoning techniques to further scale up our approach.


==> chapter_X2.tex <==
\chapter{Miscellaneous - Multi-Window-Finder: Domain Agnostic Window Size for Time Series Data}

\section{Definitions and Notation}\label{DefinitionsandNotation}
We begin by describing the necessary notation and definitions. 
The data type of interest is \textit{time series}:

\textbf{Definition 1 (Time series):} A time series \(T\) of length \(n\) is a sequence of real-valued numbers: $t_i:T=t_1,t_2,\ldots,t_n.$

 A local region of time series is called a \textit{subsequence}:
 
\textbf{Definition 2 (Subsequence):} A subsequence \(T_{i,m}\) of a time series \(T\) is a continuous ordered subset of the values from \(T\) of length \(m\) starting from position \(i\). \(T_{i,m}=t_i,t_{i+1},\ldots,t_{i+m-1}\), where \(1\le i \le n-m+1\).

\textbf{Definition 3 (Moving mean):} 
A moving mean is a calculation used to analyze data points by creating a series of averages of different subsequences in the time series.
Most of the time, moving mean is used to mitigate the effects of small fluctuations in the time series data.

\section{Related Work}\label{RelatedWork}
Many data mining tasks require window size which ought to be provided based on expert knowledge or field domain. Given the fact that window size is a crucial parameter towards optimal performance of such tasks, here we briefly discuss some of the existing research on time series window size calculation.

Madrid et al. \cite{madrid2019matrix} introduced Pan Matrix Profile (PMP), for all subsequences of all lengths, which allows for parameter-free motif discovery. Note, this algorithm uses an upper bound for the window size. In classic motif discovery algorithm, the user can run the matrix profile to find the pattern. However, matrix profile needs a window size parameter. Pan Matrix Profile runs the matrix profile for all different window sizes and since it computes the Pearson correlation, the algorithm can compare patterns of different window sizes to each other. Then it finds the motif that has highest Pearson correlation.

Also Gao et al. \cite{gao2017iterative} introduced a series of tools to allow interactive discovery of variable-length time series motifs. However, this work is different from PMP. Firstly, because they use a discretized representation of the data (for efficiency), they end up finding approximate answers. Secondly, they only return information about a small subset of the patterns, whereas PMP contains exact distances for all subsequences of all lengths.

In a similar effort, \cite{nakamura2020merlin} proposed a variant of Matrix Profile, namely MERLIN, which is suited at finding discords (i.e. subsequences of a time series that are maximally far away from their nearest neighbors) of arbitrary length in the time series.

It is worthwhile to mention the Fast Fourier Transform (FFT) can be used to find optimal window size. The FFT converts the signal from time domain into the frequency domain and vice versa. However, FFT generates a poor result when you have time-variant and non-stationary data or when working with sharp corners. As we show later for some of the time series data due to the existence of spikes, dropouts or noise FFT algorithm would generate poor results.

\section{Finding Window sizes of Time Series}\label{MltiWindowAlgorithm}
In this section we introduce Multi-Window-Finder algorithm, which allows us to find all window lengths relevant to the time series data. The assumption of this algorithm is that each behavior is repeated for couple of times.


One might say that through asking an expert or domain knowledge might be enough to find the right window size. However, human error can never undermined. Moreover, in many cases where we have a steam of data or a lot of time series, asking an expert or domain knowledge is not a scalable solution. Note that our algorithm is very efficient and fast, which can automate the burdensome and time-consuming task of determining window size.

\subsection{Multi-Window-Finder}

The intuition behind this algorithm is that the error towards moving average for any given window size will decrease as we get closer to the actual window size of time series, and increases as we get farther.

To make this clear, let us explain through an example. Suppose we have a time series of Arterial Blood Pressure (ABP) of a patient, as in Fig.~\ref{fig:ABP} (bottom). A snippet of the Arterial Blood Pressure time series is shown in  Fig.~\ref{fig:ABP} (top).

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/ABP.png}
    \caption{top) The zoom in version of the time series data bottom) The time series corresponds to Arterial Blood Pressure.}~\label{fig:ABP}
     \vspace{-0.4cm}
\end{figure}

Let us compute the moving average of this time series for different window sizes. Fig.~\ref{fig:MAABP} shows the small section of the moving averages for different window sizes. The black dashed line is the mean value of these moving averages. From the left subplots we can see that as we increase the window size of the moving average, the moving average distance to the mean (black dashed line) decreases, however, in the right subplots as we increase the window size the moving average distance to the mean increases. The right window size is the one that the moving average has the lowest distance to the mean.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/MAABP.png}
    \caption{left) The moving average corresponding to window sizes 100, 150 and 240. The black dashed line is the mean of the moving average. Right) The moving average corresponding to window sizes of 240,300 and 350. The black dashed line is the mean of the moving average.}~\label{fig:MAABP}
     \vspace{-0.7cm}
\end{figure}

From this observation we can compute the time series actual window size. First we compute the moving average for different window sizes and then we compute the distance of these moving averages from the total mean of moving average for each window which we call it moving-dist meta time series, as shown in Fig.~\ref{fig:MAW}. Next, we locate the first valley of the moving-dist meta time series, which represents the minimum window size for the time series data. Note that the next valley is almost two times bigger in size compared with the first valley and the third valley is three times bigger than the first valley and so on. Using this information, we can compute the confidence interval of the window size. First we compute the error using the standard deviation of these windows and then compute the confidence interval using error. For this time series the window size is 240 with the confidence of \% 96.


The main algorithm for finding window size is outlined in Algorithm \ref{findingwindowalgorithm}, and its subroutine that computes the moving average for different window sizes is outlined in Algorithm \ref{movingmeanalgorithm}. In Algorithm \ref{findingwindowalgorithm}, we compute all the moving averages and then we compute the residuals which would be the absolute distance of moving average from its mean value. After computing residuals, we compute local minimums and subsequently compute the window size and confidence interval. For simplicity in Algorithm \ref{findingwindowalgorithm} we set the parameter `e' which is the maximum length of window size to some large value (e.g. 1000 here). In general, we continue increasing the window size until we find at least three local minimum as shown in Fig.~\ref{fig:MAABP}, which means this algorithm is parameter free.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/MAW.png}
    \caption{Moving-dist corresponding to the time series of arterial blood pressure for different window sizes. The red dots are the local minimums. }~\label{fig:MAW}
     \vspace{-0.7cm}
\end{figure}


\begin{algorithm}
\caption{Multi-Window-Finder}\label{findingwindowalgorithm}
\hspace{-5.5cm}{\REQUIRE {\textrm{\textbf{Input:} time series $T$}}}
\\
\hspace{-3.1cm}{\ENSURE {\textrm{\textbf{Output:} window size $w$, confidence $c$}}}
\begin{algorithmic}[1]
\State $ s \xleftarrow{} 10,  e \xleftarrow{} 1000, ws \xleftarrow{} empty $  
\For {$w \xleftarrow{} ~s~ \textrm{to} ~ e$}
\State $ $\textrm{MA}$ =
$\textrm{moving-avg(T, w)}$ \textrm{~//Algroithm 2}$
\State $ $\textrm{moving-dist}$ \xleftarrow{} Sum(Log(abs($\textrm{MA}$ - mean($\textrm{MA}$ ))) $ 
\State $ ws \xleftarrow{} w$
\EndFor
\State $ $\textrm{local-min}$ =  $diff(sign(diff(moving-dist))) > 0).nonzero()[0] + 1 $ $
\For {$ $\textrm{i in local-min}$ $}
\State $ res \xleftarrow{}  ws[i]/(i+1)$
\EndFor   
\State $ w = mean($\textrm{res}$) $
\State $ c = 1 - std($\textrm{res}$) $
\State \textrm{\textbf{return}} $w, c$
% % \EndProcedure
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\caption{Moving Average}\label{movingmeanalgorithm}
% \Procedure{Build-Index }{$MTS$,$sub$}\\
\hspace{-3.1cm}{\REQUIRE {\textrm{\textbf{Input:} time series $T$, window-size $w$}}}
\\
\hspace{-3.1cm}{\ENSURE {\textrm{\textbf{Output:} moving average $\textrm{moving-avg}$}}}
\begin{algorithmic}[1]
\State $ $\textrm{moving-avg}$ = $\textrm{cumsum}[T]$ \textrm{~//cumulative sum}$
\State $\textrm{moving-avg}[w:] = \textrm{moving-avg}[w:] - \textrm{moving-avg}[:w]$
\State $ moving-avg = \textrm{moving-avg}[w-1:] / w$
\State \textrm{\textbf{return}} $\textrm{moving-avg}$
% \EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Time series with different window sizes}\label{Timeserieswithdifferentwindowsizes}
Often the time series consists of different behaviors. For example, most of the time series that is generated by human activities consist of different activities such as running, walking, cycling and etc. A data analyst might ask: \textit{How can we find window size for such a time series?} In this section, we expand our method of finding one window size to find a meta-time series that represents a variable window size for each section of time series.


For illustration of our method, we  use  PAMAP  physical  activity  monitoring  dataset \cite{ainsworth2000compendium}; which  contains  a  wide  range  of everyday  household  and fitness activities performed by a number of human subjects. The data is  generated  by  subjects  wearing  3D  inertial  measurement units (IMUs) and a heart rate (HR) monitor. This dataset has been  used  for  many  other  tasks  such  as activity  recognition, segmentation, feature extraction, and classification.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/windowmeta.png}
    \caption{The meta-time series (pink) generated by Multi-Window-Finder algorithm which corresponds to variable window sizes of time series. Time series corresponding to walking, running and playing soccer behaviors (blue). }~\label{fig:windowmeta}
     \vspace{-0.7cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/behaviors.png}
    \caption{Three instances of (left) walking, (center) running and (right) playing soccer behaviors.}~\label{fig:behaviors}
     \vspace{-0.7cm}
\end{figure}

Consider a time  series  that  represents training session of a soccer player, as in Fig~.\ref{walk_run_playspoccer_pamap}. The player initially warms up with exercises such as walking and running, and then starts to play soccer. Fig~.\ref{fig:windowmeta} (bottom) shows a time  series consisted of walking, running and finally playing soccer from a hip-mounted accelerometer collected at 100 HZ. To find the best window size for this time series, we will run Algorithm \ref{findingwindowalgorithm} for small batches of this time series. This can help us to generate a meta-time series that represents window size for each section of time series. The result is shown in Fig~.\ref{fig:windowmeta} (red). As you can see this time series has a different window size for each behavior. To compare our results with the ground truth, we extract one generic pattern from each behavior as shown in Fig~.\ref{fig:behaviors}. As you can see, our results are very close to the value of the ground truth window sizes. The capability of finding different window sizes can help us to find the better quality motifs, discords and subsequently do better with other data mining tasks.

Let us consider another example. Suppose a user wants to analyze the time series of Fig.~\ref{fig:windowmeta2}. The first question the user might ask is \textit{What is the window size of this time series so I can run motif discovery algorithm?} By randomly sampling parts of this time series, the user learns that this time series consist of one behavior. However, If the user runs Multi-Window-Finder algorithm, surprisingly it shows two different window sizes for this time series.

Fig.~\ref{fig:samplewindowmeta2} shows the zoomed in version of this time series from two different regions. The red region belongs to the beginning of the time series (staring position at 1000) and the blue snippet belongs to the last part (starting position at 150k). For visualization purposes, Fig.~\ref{fig:samplewindowmeta2} shows this two snippets on top of each other. For the period of 5000 points, one behavior in the red snippet appears ten times however the blue behavior repeats twelve times which means there are two different window sizes. The behavior of this time series has changed after some time. Note, this information provides the user with better insight of time series and this user might investigate the reason for this change.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/windowmeta2.png}
    \caption{bottom) Time series data. top) The red vector represents the results of Multi-Window-Finder algorithm. }~\label{fig:windowmeta2}
     \vspace{-0.8cm}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/samplewindowmeta2.png}
    \caption{The blue snippet corresponds to the position of 1000 and the red snippet corresponds to the position of 150k of the original time series as shown in Fig.~\ref{fig:windowmeta2}}~\label{fig:samplewindowmeta2}
     \vspace{-0.8cm}
\end{figure}

\subsection{Time Complexity}
For computing the window size, we need to compute moving mean of time series which takes $O(n)$ where $n$ is the length of time series. Given that we are running the algorithm for different window sizes, the complexity is $O(kn)$. Note, we are assuming the window size is small in comparison to $n$ which means $k$ is small.
% Also, since the time series data is an ordered value, we can use locality of the time series data to find the window size in small batches, this will allow to find more than one window size, as time series data changes over time. This is hinted to in Figure y.

% Suppose we have the following time series.
% Let us compute the moving mean of the time series for different window sizes.




\section{Experimental Evaluation}\label{ExperimentalEvaluation}
In this section, we demonstrate performance and superiority of Multi-Window-Finder through experiments. To ensure that our experiments are easy to reproduce, we have created a website that contains all code and materials for all experiments \cite{multiwindowfinder}. We used the time series collection of KDD Cup 2021 that contains 250 time series datasets. This collection contains a variety of time series related to different domains such as human behavior and health domain. Although the collection in the KDD Cup is aimed at detecting anomaly, we will use this collection for the purpose of finding window size which is needed for most anomaly detection algorithms.

% Fig~.\ref{fig:sample} shows a snippet of time series for a few datasets in this collection. For every samples we ran FFT algorithm as well as our proposed Multi-Window-Finder algorithm to find the window size as shown in Table \ref{fftandours}. FFT algorithm in some cases produces reasonable results (Time series E) however, in other cases (Time series A through D) the existence of noise, spikes or dropouts negatively impacts the output of FFT algorithm and produces inaccurate results.


Fig~.\ref{fig:sample} shows a snippet of time series for a few datasets in this collection. We ran FFT algorithm as well as  Multi-Window-Finder algorithm to find the window size as shown in Table \ref{fftandours}. As we can see from the results, the existence of noise or spikes negatively impacts the output of FFT algorithm and produces inaccurate results.

\definecolor{LightCyan}{rgb}{0.90,1,1}
\begin{table}[h]
\caption{The performance of FFT and Multi-Window-Finder algorithms.}\label{fftandours}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor{LightCyan} Time Series & Ground Truth & FFT & Multi-Window-Finder
    \\ \hline
A & 150 &  83 & 161\\ \hline
% B & 200 &  681 & 187\\ \hline
B & 100 &  930 & 105\\ \hline
% D & 165 &  83 & 161\\ \hline
% E & 200 &  218 & 202\\ \hline      
\end{tabular}
\end{center}

\end{table}
\\
\vspace{-0.3cm}



We further asked an expert in the time series domain to label window size of all the time series in this collection. This can help us to compare the results of Multi-Window-Finder algorithm against the ground truth. We measure the performance of Multi-Window-Finder algorithm using the following formula.
    
% \[
% error = \frac{ abs(Window_{ground\ truth} - Window)}{Window_{ground\ truth}}
% \]

\[
    success\_rate= 
\begin{cases}
    1&  \frac{ abs(\textrm{Window}_{\textrm{ground\ truth}} - \textrm{Window})}{\textrm{Window}_{\textrm{ground\ truth}}})\leq 0.5\\
    0              & \text{otherwise}
\end{cases}
\]

% In computing error, we calculated the absolute error distance of the output of our Multi-Window-Finder versus the ground truth for every time series, and then we determined the total error by summing up all error values.

For the success rate, if the output of our Multi-Window-Finder is close to the ground truth window, then we count it as success, otherwise we count it as no success. Then we sum up all successes and report the total success for the whole collection. The results are shown in Table \ref{performance}.


\definecolor{LightCyan}{rgb}{0.90,1,1}

\begin{table}[h]
\caption{Total success rate of FFT and Multi-Window-Finder algorithms.}\label{performance}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\rowcolor{LightCyan} KDD cup dataset  & FFT  & Multi-Window-Finder
    \\ \hline
   250 time series &  171 & 190\\ \hline
\end{tabular}
\end{center}
\end{table}
\vspace{-0.3cm}

\captionsetup[figure]{font=small,skip=0pt}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25,width=0.9\columnwidth]{figures/sample.png}
    \caption{Two snippets of time series dataset from KDD cup. top) data with drop out bottom) data with noise.}~\label{fig:sample}
    \vspace{-0.7cm}
\end{figure}

As you can see the results are very promising. Out of 250 time series, in 190 of these time series Multi-Window-Finder algorithm is accurate. We further investigated the discrepancy between the results of Multi-Window-Finder algorithm and the ground truth. For some of the cases, the time series has more than one window size which reporting just one was not ideal. In other cases, the Multi-Window-Finder result is twice bigger than the ground truth and we do not know what the correct size for these time series.
% \subsection{Robustness Test}\label{RobustnessTest}
% In this section, we examine robustness of Multi-Window-Finder to the effect of adding random noise to time series data. 




% . The ability to detect periodicity in time series is
% fundamental when it comes to forecasting [7]

%  However, periodicities detection is not easy and has been greatly
% studied in the existing literature, but most of current techniques are unable to
% detect periodicities without the need of preprocessing data [14] or have trouble
% detecting multiple periodicities [13]. This paper is organised as follow: we first
% present the Fourier transform and the Autoperiod algorithm [13] used to detect
% periodicities in a signal. Then we propose a new fully automated method, named
% Clustered Filtered Detrended Autoperiod (CFD-Autoperiod), which also combines the advantages of frequency domain and time domain while being robust
% to noise and able to handle multi periodicities. T


\section{Discussion and Conclusions}\label{DiscussionandConclusions}

We have introduced Multi-Window-Finder algorithm which enables the user to find an appropriate window size for the time series. In addition, the expanded version of this algorithm is able to find a variable window size for time series data. Window size is a parameter that is needed for many of the algorithms in data mining discovery analysis and in many cases it is given by an expert of the domain.
Using Multi-Window-Finder algorithm we are able to make these algorithms, parameter-free. In future work, we want to expand this algorithm to handle multi dimensional time series data and test on more dataset of time series data.
